Towards Large Scale Geostatistical Methane Monitoring with Part-based Object Detection

Object detection is one of the main applications of computer vision in remote sensing imagery. Despite its increasing availability, the sheer volume of remote sensing data poses a challenge when detecting rare objects across large geographic areas. Paradoxically, this common challenge is crucial to many applications, such as estimating environmental impact of certain human activities at scale. In this paper, we propose to address the problem by investigating the methane production and emissions of bio-digesters in France. We first introduce a novel dataset containing bio-digesters, with small training and validation sets, and a large test set with a high imbalance towards observations without objects since such sites are rare. We develop a part-based method that considers essential bio-digester sub-elements to boost initial detections. To this end, we apply our method to new, unseen regions to build an inventory of bio-digesters. We then compute geostatistical estimates of the quantity of methane produced that can be attributed to these infrastructures in a given area at a given time.

==> data/histograms_anomaly.tex <==
\begin{figure}[!t]
    \raggedleft
    %\centering
    %
    % First subfigure
    \begin{subfigure}[b]{0.4\columnwidth}
        \centering
        % -- First TikZ or includegraphics code --
        \begin{tikzpicture}[baseline, trim left]
            \begin{axis}[
                scale only axis,
                axis line style={draw=none},
                axis x line=bottom, 
                axis y line=left,
                width=\linewidth*0.85,
                height=\linewidth*0.75,
                %scale=0.1,
                symbolic x coords={-0.3,0,1,2,3,4,5,6}, % Keeps the x-axis symbolic
                xtick=data,
                ymin=0,
                xmin=-0.3,
                ylabel={Frequency},
                ylabel style={at={(-0.35,0.8)}, anchor=east},
                %ylabel style={yshift=-20pt},
                xlabel={Tank Count ($N_t$)},
                legend style={font=\small, at={(0.98,0.98)}, anchor=north east},
                bar width=4pt,
                enlarge x limits=-5,
                tick label style={font=\small},
                label style={font=\small},
                legend style={font=\small},
                title style={font=\small},
            ]
                % BARS (New Values for Tanks)
                \addplot[ybar, fill=blue, opacity=0.3] 
                    coordinates {(0,0.88376) (1,0.08587) (2,0.01811) (3,0.00611) (4,0.00287) 
                                 (5,0.00137) (6,0.00072)};
                
                % LINE PLOT (New Values for Tanks)
                \addplot[mark=*, mark size=2pt, red, thick, solid] 
                    coordinates {(0,0.59978) (1,0.30660) (2,0.07837) (3,0.01335) (4,0.00171) 
                                 (5,0.00017) (6,0.00001)};

                \draw[red, thick] (axis description cs:0.45,0.95) 
                      -- (axis description cs:0.55,0.95)
                      node[anchor=west, black] {Poisson};
                \filldraw[red] (axis description cs:0.50,0.95) circle (1.5pt);
                % \legend{True Values, Poisson Approximation}
            \end{axis}
        \end{tikzpicture}
        %\caption{Tanks}
        \label{fig:tanks_anomaly}
    \end{subfigure}
    \hspace{3mm}
    %\hfill{}
    % Second subfigure
    \begin{subfigure}[b]{0.4\columnwidth}
        \centering
        % -- Second TikZ or includegraphics code --
        \begin{tikzpicture}[baseline, trim left]
            \begin{axis}[
                scale only axis,
                axis x line=bottom, 
                axis y line=left,
                axis line style={draw=none},
                width=\linewidth*0.85,
                height=\linewidth*0.75,
                symbolic x coords={-0.3,0,1,2,3,4,5,6}, % Keeps the x-axis symbolic
                xtick=data,
                ymin=0,
                xmin=-0.3,
                xlabel={Pile Count ($N_p$)},
                legend style={font=\small, at={(0.98,0.98)}, anchor=north east},
                bar width=4pt,
                enlarge x limits=0.0,
                tick label style={font=\small},
                label style={font=\small},
                legend style={font=\small},
                title style={font=\small},
                %scaled ticks=false, 
                %y tick scale label code/.code={},
                yticklabel style={/pgf/number format/fixed}, 
            ]
                % Bars
                \addplot[ybar, fill=blue, opacity=0.3] 
                    coordinates {(0,0.93005) (1,0.05367) (2,0.01218) (3,0.00303) (4,0.00075) 
                                 (5,0.00022) (6,0.00007)};
                
                % LINE PLOT (New Values for Piles)
                \addplot[mark=*, mark size=2pt, red, thick, solid] 
                    coordinates {(0,0.57280) (1,0.31918) (2,0.08893) (3,0.01652) (4,0.00230) 
                                 (5,0.00026) (6,0.00002)};
            \end{axis}
        \end{tikzpicture}
        %\caption{Piles}
        \label{fig:piles_anomaly}
    \end{subfigure}

    \caption{Tanks and Piles counts in False Detections}
    \label{fig:comparison_anomaly}
\end{figure}

==> data/tiling.tex <==
\begin{figure}[ht]
    \centering
    \begin{tikzpicture}
        % Define primary axis (Probability of Detection)
        \begin{axis}[
            width=\linewidth*0.9, height=\linewidth*0.6,
            xlabel={$H/S$},
            ylabel={Uncut probability},
            ylabel style={yshift=-2pt}, % -12
            ymin=0.8, ymax=1.05,
            xmin=0.8, xmax=1.0,
            axis y line*=left,
            axis x line=bottom,
            tick label style={font=\small},
            label style={font=\small},
            legend style={font=\small},
            title style={font=\small},
            legend style={at={(0.98,0.98)}, anchor=north east, fill=none, draw=none}
        ]
            % Probability of Detection
            \addplot[blue, thick, mark=s, mark options={fill=blue}, line width=1.2pt] coordinates {
                (0.8, 1.0)
                (0.8105263157894738, 1.0)
                (0.8210526315789474, 1.0)
                (0.8315789473684211, 1.0)
                (0.8421052631578948, 1.0)
                (0.8526315789473684, 1.0)
                (0.8631578947368421, 1.0)
                (0.8736842105263158, 1.0)
                (0.8842105263157896, 1.0)
                (0.8947368421052632, 1.0)
                (0.9052631578947369, 0.991)
                (0.9157894736842105, 0.9708)
                (0.9263157894736842, 0.9484)
                (0.9368421052631579, 0.931)
                (0.9473684210526316, 0.9126)
                (0.9578947368421052, 0.8906)
                (0.968421052631579, 0.8606)
                (0.9789473684210527, 0.8564)
                (0.9894736842105263, 0.828)
                (1.0, 0.8162)
            };
            \addlegendentry{Uncut probability}
        \end{axis}
        
        % Define secondary axis (Number of Passes)
        \begin{axis}[
            width=\linewidth*0.9, height=\linewidth*0.6,
            xlabel={},
            ylabel={Inferences per pixel}, 
            ylabel style={at={(1.15,0.0)}, anchor=west}, % 1.4 0.2
            ymin=1.0, ymax=1.6,
            xmin=0.8, xmax=1.0,
            axis y line*=right,
            axis x line=bottom,
            tick label style={font=\small},
            label style={font=\small},
            legend style={font=\small},
            title style={font=\small},
            xtick=\empty,
            xticklabels=\empty,
            legend style={at={(0.02,0.02)}, anchor=south west, draw=none}
        ]
            % Number of Passes
            \addplot[Orange, thick, mark=s, line width=1.2pt] coordinates {
                (0.8, 1.5625)
                (0.8105263157894738, 1.522179119581717)
                (0.8210526315789474, 1.4833990795529255)
                (0.8315789473684211, 1.446082358596379)
                (0.8421052631578948, 1.41015625)
                (0.8526315789473684, 1.37555250723975)
                (0.8631578947368421, 1.342207019631172)
                (0.8736842105263158, 1.3100595151691101)
                (0.8842105263157896, 1.2790532879818592)
                (0.8947368421052632, 1.249134948096886)
                (0.9052631578947369, 1.2202541914548406)
                (0.9157894736842105, 1.1923635883207822)
                (0.9263157894736842, 1.1654183884297524)
                (0.9368421052631579, 1.139376341371039)
                (0.9473684210526316, 1.1141975308641974)
                (0.9578947368421052, 1.0898442217123536)
                (0.968421052631579, 1.0662807183364837)
                (0.9789473684210527, 1.043473233899873)
                (0.9894736842105263, 1.0213897691263016)
                (1.0, 1.0)
            };
            \addlegendentry{Inferences per pixel}
        \end{axis}
    \end{tikzpicture}
    \caption{Uncut probability and Inferences per pixel as a Function of Hop Length Fraction (for 1km x 1km tiles)}
    \label{fig:prob_vs_hop}
\end{figure}

==> imgs/ign_vs_spot.tex <==
\newcommand{\igncrop}{220pt}  % Adjust this parameter for IGN cropping
\newcommand{\spotcrop}{330pt}   % Adjust this parameter for SPOT cropping * 1.5

\begin{figure}
    \centering
    \begin{tabular}{cc}
        \includegraphics[trim=\igncrop{} \igncrop{} \igncrop{} \igncrop{},clip,width=0.45\linewidth]{imgs/ign_vs_spot/ign_0012.png} & 
        \includegraphics[trim=\spotcrop{} \spotcrop{} \spotcrop{} \spotcrop{},clip,width=0.45\linewidth]{imgs/ign_vs_spot/spot_0009.png} \\
        \includegraphics[trim=\igncrop{} \igncrop{} \igncrop{} \igncrop{},clip,width=0.45\linewidth]{imgs/ign_vs_spot/ign_0015.png} & 
        \includegraphics[trim=\spotcrop{} \spotcrop{} \spotcrop{} \spotcrop{},clip,width=0.45\linewidth]{imgs/ign_vs_spot/spot_0011.png} \\
        %\includegraphics[trim=\igncrop{} \igncrop{} \igncrop{} %\igncrop{},clip,width=0.45\linewidth]{imgs/ign_vs_spot/ign_0019.png} & 
        %\includegraphics[trim=\spotcrop{} \spotcrop{} \spotcrop{} %\spotcrop{},clip,width=0.45\linewidth]{imgs/ign_vs_spot/spot_0013.png} \\
    \end{tabular}
    \caption{\textbf{Comparison of aerial and satellite datasets.} IGN data is shown on the left and SPOT6-7 images on the right.}
    \label{fig:ign_spot}
\end{figure}


==> imgs/img_maps_normandie.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/heat_maps_1/normandie_fused_map.pdf}
    \caption{\textbf{Fused map showing both the heat map of bio-digester detections and the inventory per department in Normandie}, including Unclear detections and \cite{methanisation_orne_2024} database.}
    \label{fig:maps_normandie}
\end{figure}

==> imgs/imgs_examples.tex <==


\begin{figure*}[]
    \centering

    % Images in one row with captions below , trim=300 300 300 300, clip
    \begin{tabular}{cccc}
        \includegraphics[height=3cm, trim=120 120 120 120, clip]{imgs/imgs_examples/unclear_1.png} &
        \includegraphics[height=3cm, trim=120 120 120 120, clip]{imgs/imgs_examples/unclear_8.png} &
        \includegraphics[height=3cm, trim=120 120 120 120, clip]{imgs/imgs_examples/bg_4.png} &
        \includegraphics[height=3cm, trim=120 120 120 120, clip]{imgs/imgs_examples/bg_6.png} \\
        (a) Unclear & (b) Unclear & (c) False positive & (d) False positive
    \end{tabular}

    \vspace{-1em}
    \begin{center}
        \begin{tikzpicture}
            \newcommand{\rectwidth}{0.6}  % Width of rectangles
            \newcommand{\rectheight}{0.3}  % Height of rectangles

            % Bio-digester
            \draw[fill={rgb,255:red,237;green,23;blue,232}, draw=black] (0,0) rectangle (\rectwidth,\rectheight);
            \node[right] at (\rectwidth*1.3,\rectheight/2) {\textbf{Bio-digester}};
        
            % Piles
            \draw[fill={rgb,255:red,255;green,173;blue,30}, draw=black] (5,0) rectangle ({5+\rectwidth},\rectheight);
            \node[right] at (5+\rectwidth*1.3,\rectheight/2) {\textbf{Piles}};
        
            % Tanks
            \draw[fill={rgb,255:red,0;green,69;blue,255}, draw=black] (10,0) rectangle ({10+\rectwidth},\rectheight);
            \node[right] at (10+\rectwidth*1.3,\rectheight/2) {\textbf{Tanks}};
        \end{tikzpicture}
    \end{center}
    \vspace{-1em}

    \caption{Example of detections classified as Unclear (a), (b) and False positive (c), (d)}
    \label{fig:imgs_examples}

\end{figure*}

==> maps/sheme_tile.tex <==
\begin{figure}[ht]
  \centering
  \begin{tikzpicture}[scale=3]
    % Outer image boundary of size S + H (here S=1, H=0.8)
    % \draw[thick] (0,0) rectangle (1.8,1.8);

    % Tiles with size S=1 and hop H=0.8
    \draw[gray!60, dashed] (0,0) rectangle (1,1);
    \draw[gray!60, dashed] (0.8,0) rectangle (1.8,1);
    \draw[gray!60, dashed] (0,0.8) rectangle (1,1.8);
    \draw[gray!60, dashed] (0.8,0.8) rectangle (1.8,1.8);

    % Tile labels
    \node at (0.5,1.65-0.2) {Tile 1};
    \node at (1.3,1.65-0.2) {Tile 2};
    \node at (0.5,0.85-0.2) {Tile 3};
    \node at (1.3,0.85-0.2) {Tile 4};

    % Hop length arrow
    \draw[<->, thick] (0,-0.1) -- (0.8,-0.1) node[midway, below] {$H = 0.8S$};

    % Good object inside Tile 1 (green)
    \draw[green, thick] (0.15,0.95) rectangle ++(0.7,0.4);

    % Bad object crossing Tile 3 & Tile 4 (red)
    \draw[red, thick] (0.6,0.1) rectangle ++(0.5,0.4);
  \end{tikzpicture}
  \caption{Illustration of 4 overlapping tiles with hop length $H=0.8S$. The green box is fully inside Tile 1, and the red box straddles Tiles 3 and 4.}
  \label{fig:tilescheme}
\end{figure}

